On the Cost of Concurrency in Hybrid Transactional Memory

State-of-the-art \emph{software transactional memory (STM)} implementations achieve good performance by carefully avoiding the overhead of \emph{incremental validation} (i.e., re-reading previously read data items to avoid inconsistency) while still providing \emph{progressiveness} (allowing transactional aborts only due to \emph{data conflicts}). Hardware transactional memory (HTM) implementations promise even better performance, but offer no progress guarantees. Thus, they must be combined with STMs, leading to \emph{hybrid} TMs (HyTMs) in which hardware transactions must be \emph{instrumented} (i.e., access metadata) to detect contention with software transactions. We show that, unlike in progressive STMs, software transactions in progressive HyTMs cannot avoid incremental validation. In fact, this result holds even if hardware transactions can \emph{read} metadata \emph{non-speculatively}. We then present \emph{opaque} HyTM algorithms providing \emph{progressiveness for a subset of transactions} that are optimal in terms of hardware instrumentation. We explore the concurrency vs. hardware instrumentation vs. software validation trade-offs for these algorithms. Our experiments with Intel and IBM POWER8 HTMs seem to suggest that (i) the \emph{cost of concurrency} also exists in practice, (ii) it is important to implement HyTMs that provide progressiveness for a maximal set of transactions without incurring high hardware instrumentation overhead or using global contending bottlenecks and (iii) there is no easy way to derive more efficient HyTMs by taking advantage of non-speculative accesses within hardware.

==> conc.tex <==
%!TEX root = htm.tex
\section{Concluding remarks}
\label{sec:conc}

==> hybridnorec.tex <==
\begin{algorithm*}[!h]
\caption{HybridNorec HyTM implementation; code for $T_k$ by process $p_i$}
\label{alg:inswrite3}
\vspace{-1mm}
\noindent\lstset{style=customc}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}[frame=none,firstnumber=1,mathescape=true]
//\textbf{Shared objects}
    L, global single-bit lock

//\textbf{Code for fast-path transactions}
start$_k$()
    if esl==1
	return A$_k$

read$_k$(X$_j$)
    ov$_j$ := v$_j$ //\medcom cached read
    return ov$_j$

write$_k$(X$_j$, v)
    v$_j$ := v //\medcom cached write
    return OK

try$C_k$()
    if $\Wset(T_k)= \emptyset$ then
	return C$_k$
    l:= gsl
    if l $\mathrel{\&} 1$ then
	return A_$k$
    gsl:=l+2
    return commitCache$_i$() //\medcom returns $C_k$ or $A_k$

Function: $\lit{validate}()$}
    currGSL:=gsl
    if sl == currGSL then
	return true
    while true
        while currGSL $\mathrel{\&} 1$
	    currGSL:=gsl
	if $\exists$ X$_j$ $\in$ Rset(T$_k$):ov$_j$ $\neq$ X$_j$ then
	    return false
    	if gsl == currGSL then
	    sl:=currGSL
	    return true

\end{lstlisting}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}[frame=none,firstnumber=last,mathescape=true]
//\textbf{Code for slow-path transactions}
start$_k$()
    while sl $\mathrel{\&} 1$
	sl:= gsl

read$_k$(X$_j$)
    if X$_j$ $\in \Wset(T_k)$ then
	return $\Wset(T_k).\lit{locate}(X_j)$ 
    ov$_j$ := v$_j$ //\medcom cached read
    Rset(T$_k$) := Rset(T$_k$)$\cup${X$_j$,or$_j$} //\label{line:rset}
    if $\neg$ validate() then 
	return A$_k$
    return ov$_j$

write$_k$(X$_j$, v)
    v$_j$ := v //\medcom cached write
    return OK

tryC$_k$()
    if Wset(T$_k$) = $\emptyset$ then return $C_k$
    while sl $\mathrel{\&} 1$ or $\neg\ms{gsl}$.CAS($sl$, $sl+1$)  
          sl:= gsl
    esl:=1
    if validate() then
        esl:=0
        gsl:=gsl+1
        return $A_k$
    for each X$_j \in$ Wset(T$_k$) do v$_j$ := nv$_j$
    esl:=0
    gsl:=gsl+1
    return $C_k$
\end{lstlisting}
\end{minipage}
\vspace{-1mm}
\end{algorithm*}

% \begin{algorithmic}[1]
%   	\begin{multicols}{2}
%   	{
%   	\footnotesize
% 	\Part{Shared objects}{
% 		\State $\ms{gsl}$, global sequence lock 
% 		%\Statex ~~~~~allows reads, writes
% 		\State $\ms{esl}$, extra sequence lock-bit
% 		
% 	}\EndPart	
%  	\Statex
%  	\Part{Process local objects}{
%  		\State $\ms{sl}_i$, process $p_i$'s local sequence lock
%  		
%  	}\EndPart
% 	\Statex
% 	\textbf{Code for fast-path transactions}	
% 	\Statex
% 	\Part{$\textit{start}_k()$}{
% %		\State $ \ms{l}   \gets \Read(\ms{esl})$
% 		\If {$\Read(\ms{esl})$}
% 		  \Return $A_k$ \EndReturn
% 		\EndIf
% 		
% 	}\EndPart
% 	\Statex
% 	%\Comment{In general, would it better to buffer writes in tryC?}
% 	\Part{$\textit{read}_k(X_j)$}{\quad\Comment{fast-path}
% 		
% 		\State $\textit{ov}_j := v_j.\Read()$ \Comment{cached read} 
% 		
% 		\Return $\textit{ov}_j$ \EndReturn
% 		
%    	 }\EndPart
% 	\Statex
% 	\Part{$\textit{write}_k(X_j,v)$}{\quad\Comment{fast-path}
% 	
% 	\State $v_j.\Write(v)$ \Comment{cached write}
% 	\Return $\ok$ \EndReturn
% 		
%    	}\EndPart
% 	\Statex
% 	
% 	%\Statex	
% 	\Part{$\textit{tryC}_k$()}{\quad\Comment{fast-path}
% 		%\Return $C_k$ \EndReturn
% 		\If{$\Wset(T_k)= \emptyset$}
% 			\Return $C_k$ \EndReturn 
% 		\EndIf
% 		\State $ \ms{l}   \gets \Read(\ms{gsl})$
% 		\If {$\ms{l} \mathrel{\&} 1$}
% 		  \Return $A_k$ \EndReturn
% 		\EndIf
% 		\State $\ms{gsl}.\lit{write}(l+2)$
% 		\State $\ms{commit-cache}_i$ \Comment{returns $C_k$}
% 		
%    		
%    	 }\EndPart		
%    	 \Statex
% 	\Statex
% 	\textbf{Code for slow-path transactions}
% 	\Statex
% 	\Part{$\textit{start}_k()$}{
% 		\While {$\ms{sl} \mathrel{\&} 1$}
% 		  \State $ \ms{sl}   \gets \Read(\ms{gsl})$
% 		\EndWhile
% 		
% 	}\EndPart
% 	\Statex
% 	\Part{\Read$_k(X_j)$}\quad\Comment{slow-path}{
% 		  \If{$X_j\in \Wset(T_k)$}
% 		    \Return $\Wset(T_k).\lit{locate}(X_j)$ \EndReturn
% 		  \EndIf
% 		  \State $\textit{ov}_j := \Read(v_j)$ 
% 		  
% 		  \State $\Rset(T_k) := \Rset(T_k)\cup\{X_j,or_j\}$
% 		  \If{$\neg \lit{validate}()$}
% 			
% 			\Return $A_k$ \EndReturn
% 		  \EndIf
% 		  \Return $\textit{ov}_j$ \EndReturn
% 	
%    	 }\EndPart
%    	\newpage
% 	\Part{\Write$_k(X_j,v)$}\quad\Comment{slow-path}{
% 		
% 			\State $\textit{nv}_j := v$
% 			\State $\Wset(T_k) := \Wset(T_k)\cup\{X_j,nv_j\}$
% 			\Return $\ok$ \EndReturn
% 		
%    	}\EndPart
% 	\Statex
% 	
% 	%\Statex	
% 	\Part{\TryC$_k$()}\quad\Comment{slow-path}{
% 		\If{$\Wset(T_k)= \emptyset$}
% 			\Return $C_k$ \EndReturn 
% 		\EndIf
% 		
% 		\While{$\ms{sl} \mathrel{\&} 1 \mbox{ \textbf{or} } \neg\ms{gsl}$.CAS($sl$, $sl+1$)} \Comment{Lock gsl} 
%           \State $\ms{sl} \gets \Read(\ms{gsl})$
% 		\EndWhile
% 		\State $\ms{esl}.\lit{write}(1)$
% 		\If{$\neg\lit{validate}()$}
%     		\State $\ms{esl}.\lit{write}(0)$
% 			\State $\ms{gsl}.\lit{write}(\lit{read}(\ms{gsl})+1)$
% 			\Return $A_k$ \EndReturn
% 		\EndIf
% 		\ForAll{$X_j \in \Wset(T_k)$}
% 	 		 \State  $v_j.\lit{write}(\textit{nv}_j)$
% 		\EndFor
% 		\State $\ms{esl}.\lit{write}(0)$
% 		\State $\ms{gsl}.\lit{write}(\lit{read}(\ms{gsl})+1)$
%   		\Return $C_k$ \EndReturn
%    	 }\EndPart		
% 	\Statex
% 	\Part{Function: $\lit{validate}()$}{
%         \State $\ms{currGSL} \gets \Read(\ms{gsl})$
% 		\If{$\ms{sl} = \ms{currGSL}$}
%             \Return $\true$ \EndReturn
%         \EndIf
%         \While{$true$}
%             \While{$\ms{currGSL} \mathrel{\&} 1$}
%                 \State $\ms{currGSL} \gets \Read(\ms{gsl})$
%             \EndWhile
%     		\If{$\exists X_j \in Rset(T_k)$:$(\textit{ov}_j \neq \Read(X_j))$}
%     			\Return $\false$ \EndReturn
%     		\EndIf
%             \If{$\Read(gsl) = \ms{currGSL}$}
%                 \State $\ms{sl} \gets \ms{currGSL}$
%         		\Return $\true$ \EndReturn
%             \EndIf
%         \EndWhile
% 	}\EndPart
% 	
% % 	
% 	}
% 	\end{multicols}
%   \end{algorithmic}
% \end{algorithm*}


==> middle.tex <==
\begin{algorithm*}[!h]
\caption{Transformation for opaque HyTM $\mathcal{M}$ to include a fast fast-path; code for $T_k$ by process $p_i$}
\label{alg:middle}
\vspace{-1mm}
\noindent\lstset{style=customc}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}[frame=none,firstnumber=1,mathescape=true]
//\textbf{Shared objects}
    F, fetch-and-increment object
    
//\textbf{Code for slow-path transactions}
tryC$_k$()
    if $\Wset(T_k)= \emptyset$ then
	return C$_k$  
    $F.\lit{fetch-add}(1)$
    //\textbf{Invoke updating slow-path tryC$_k$(); let $r_k$ be the response}
    $F.\lit{fetch-add}(-1)$
    return r$_k$ 
\end{lstlisting}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{lstlisting}[frame=none,firstnumber=last,mathescape=true]
//\textbf{Code for fast fast-path transactions}
start$_k$()
    if F $\neq 0$ then //\medcom cached read
	return A$_k$

read$_k$(X$_j$)
    ov$_j$ := v$_j$ //\medcom cached read 
    return ov$_j$
		
write$_k$(X$_j$,v)
    v$_j$:=v  //\medcom cached write
    return ok

tryC$_k$()
    commit-cache$_i$ //\medcom returns C$_k$ or A$_k$
\end{lstlisting}
\end{minipage}
\end{algorithm*}



% \begin{algorithmic}[1]
%   	\begin{multicols}{2}
%   	{
%   	\footnotesize
% 	\Part{Shared objects}{
% 		%\State $v_j$, for each t-object $X_j$ 
% 		\State $F$, fetch-and-increment object
% 		
% 	}\EndPart	
%  	\Statex
%  	\Statex
%  	\textbf{Code for slow-path transactions}
% 	\Statex
% 	\Part{$\textit{tryC}_k$()}{\quad\Comment{slow-path}
% 		\If{$\Wset(T_k)= \emptyset$}
% 			\Return $C_k$ \EndReturn 
% 		\EndIf
% 		\State $F.\lit{fetch-add}(1)$
% 		\State \textbf{Invoke updating slow-path $\TryC_k()$; let $r_k$ be the response}
% 		
% 		\State $F.\lit{fetch-add}(-1)$
% 		\Return $r_k$ \EndReturn
%    		
%    	 }\EndPart		
% 	\newpage
% 	\textbf{Code for fast fast-path transactions}	
% 	\Statex
% 	\Part{$\textit{start}_k()$}{
% 		
% 		\If{$\Read(\ms{F}) \neq 0$} \Comment{cached read}
% 		  \Return $A_k$ \EndReturn
% 		\EndIf
% 		
% 	}\EndPart
% 	\Statex
% 	%\Comment{In general, would it better to buffer writes in tryC?}
% 	\Part{$\textit{read}_k(X_j)$}{\quad\Comment{fast fast-path}
% 		
% 		\State $\textit{ov}_j := v_j.\Read()$ \Comment{cached read} 
% 		
% 		\Return $\textit{ov}_j$ \EndReturn
% 		
%    	 }\EndPart
% 	\Statex
% 	\Part{$\textit{write}_k(X_j,v)$}{\quad\Comment{fast fast-path}
% 	
% 	\State $v_j.\Write(v)$ \Comment{cached write}
% 	\Return $\ok$ \EndReturn
% 		
%    	}\EndPart
% 	\Statex
% 	
% 	%\Statex	
% 	\Part{$\textit{tryC}_k$()}{\quad\Comment{fast fast-path}
% 		%\Return $C_k$ \EndReturn
% 		\State $\ms{commit-cache}_i$ \Comment{returns $C_k$ or $A_k$}
% 		
%    		
%    	 }\EndPart		
%    	   	
% 	
% 	}
% 	\end{multicols}
%   \end{algorithmic}
% \end{algorithm*}


==> ob01.tex <==
\begin{tikzpicture}
\node (w2) at (10,0) [] {};
\node (w1) at (10,-2) [] {};
\node (w3) at (18,-2) [] {};


\draw (w2) node [below] {\small {$W_2(X,v)$}};

\draw (w1) node [below] {\small {$W_1(X,v)$}};
%\draw (w1) node [below] {\tiny {$T_1$ commits}};

\node[draw,align=left] at (10,1) {{\large Fast-Path}};
\node[draw,align=left] at (10,-1) {{\large Slow-Path}};

\begin{scope}   
\draw [|-,thick] (8,0) node[left] {$T_2$} to (10,0);
\draw [-,dashed] (10,0) to (11.8,0);
\draw [|-|,thick] (8,-2) node[left] {$T_1$} to (12,-2);
\draw [-,dotted] (12.2,-2.5)  to (12.2,1) node[right] {$E$};
\end{scope}
%
\node[draw,align=right] at (17,.5) {\large {Aborted or incomplete}\\ {\large fast-path transaction $T_2$}};
%
\node[draw,align=right] at (3,1.8) {\rule{6mm}{1pt} \large {direct accesses}};
\node[draw,align=right] at (3,1) {\rule{2mm}{1pt} \rule{2mm}{1pt} \large{cached accesses}};

%
\end{tikzpicture}


==> ob11.tex <==
\begin{tikzpicture}

\node (w1) at (11,-2) [] {};
\node (w2) at (10,0) [] {};

\draw (w2) node [below] {\small {$W_2(X,v)$}};

\draw (w1) node [below] {\small {$W_1(X,v)$}};
%\draw (w1) node [below] {\tiny {$T_1$ commits}};

\node[draw,align=left] at (11,1) {{\large Fast-Path}};
\node[draw,align=left] at (11,-1) {{\large Slow-Path}};

\begin{scope}   
\draw [|-|,thick] (9,-2) node[left] {$T_1$} to (13,-2);
\draw [|-,thick] (9,0) node[left] {$T_2$} to (11,0);
\draw [-,dotted] (13.2,-2.5)  to (13.2,1) node[right] {$E'$};
\end{scope}
%
%
\end{tikzpicture}


==> prog-fp-sp-optimized.tex <==
\begin{algorithm}[!h]
\caption{Progressive fast-path and slow-path opaque HyTM implementation that provides invisible reads; code for transaction $T_k$}
\label{alg:inswrite}
\begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{
  	\footnotesize
	\Part{Shared objects}{
		\State $v_j \in \mathbb{D}$, for each t-object $X_j$ 
		\Statex ~~~~~allows reads, writes and cas
		%\State $L[i]$, a multi-trylock object for transaction $T_i$ 
		\State $r_{j} \in \mathbb{M}$, for each t-object $X_j$
		\Statex ~~~~~allows reads, writes and cas
		%\State implemented from reads and writes
		%\State $L$, multi-trylock
	}\EndPart	
	\Statex
	\Part{Local objects}{
		\State $\ms{Lset}(T_k) \subseteq \Wset(T_k)$, initially empty
		\State $\ms{Oset}(T_k) \subseteq \Wset(T_k)$, initially empty
		\State Integer counter for ABA, $k\in \mathbb{N}$, initially $0$
		\Statex ~~~~~increment at start of transaction
	}\EndPart
	\Statex
	\textbf{Code for slow-path transactions}
	\Statex
	\Part{\Read$_k(X_j)$}\quad\Comment{slow-path}{
		\If{$X_j \not\in \Rset_k$}
		  \State $[\textit{ov}_j,k_j] := \Read(v_j)$ 
		  \State $\Rset(T_k) := \Rset(T_k)\cup\{X_j,[\textit{ov}_j,k_j]\}$ 
		  \If{$r_j\neq 0$} 
		    \Return $A_k$ \EndReturn
		  \EndIf
		  \If{$\exists X_j \in Rset(T_k)$:$(\textit{ov}_j,k_j)\neq \Read(v_j)$} 
			\Return $A_k$ \EndReturn
		  \EndIf

		  \Return $\textit{ov}_j$ \EndReturn
		\Else
		    
		  \State $\textit{ov}_j :=\Rset(T_k).\lit{locate}(X_j)$
		  \Return $\textit{ov}_j$ \EndReturn
		\EndIf
   	 }\EndPart
	\Statex
	\Part{\Write$_k(X_j,v)$}\quad\Comment{slow-path}{
		
			\State $(\textit{ov}_j,k_j) := \Read(v_j)$
			\State $\textit{nv}_j := v$
			\State $\Wset(T_k) := \Wset(T_k)\cup\{X_j,[\textit{ov}_j,k]\}$
			\Return $\ok$ \EndReturn
		
   	}\EndPart
	\Statex
	
	%\Statex	
	\Part{\TryC$_k$()}\quad\Comment{slow-path}{
		\If{$\Wset(T_k)= \emptyset$}
			\Return $C_k$ \EndReturn 
		\EndIf
		\State locked := $\lit{acquire}(\Wset(T_k))$
		\If{$\neg$ locked}  
	 		\Return $A_k$ \EndReturn
	 	\EndIf
		\If{$\lit{isAbortable}()$} 
			\State $\lit{release}( \ms{Lset}(T_k))$ 
			\Return $A_k$ \EndReturn
		\EndIf
		\ForAll{$X_j \in \Wset(T_k)$}
	 		\State  $v_j.\lit{write}([\textit{nv}_j,k])$
			 
	 	\EndFor		
		\State $\lit{release}(\Wset(T_k))$   
   		\Return $C_k$ \EndReturn
   	 }\EndPart		
	 
 	\newpage
 	\Part{Function: $\lit{acquire}(Q$)}{
   		\ForAll{$X_j \in Q$}	
			\If{$r_j.\lit{cas}(0,1)$} 
			  \State $\ms{Lset}(T_k) := \ms{Lset}(T_k)\cup \{X_j\}$
			\Else
			  \State $\lit{release}(\ms{Lset}(T_k))$
			  \Return $\false$ \EndReturn
			\EndIf
			
		\EndFor
		
		\Return $\true$ \EndReturn 
	}\EndPart		
	 \Statex
	 \Part{Function: $\lit{release}(Q)$}{
  		\ForAll{$X_j \in Q$}	
 			\State $r_j.\Write(0)$ 
		\EndFor
		%\State $Rset_k:=Wset_k:=\emptyset$
		\Return $ok$ \EndReturn
	}\EndPart
	
	\Statex
	
	\Part{Function: $\lit{undo}(\ms{Oset}(T_k))$}{
		\ForAll{$X_j \in \ms{Oset}(T_k)$}
		    \State $v_j.\lit{cas}([nv_j,k],[ov_j,k_j])$
		 \EndFor
		\State $\lit{release}( \ms{Wset}(T_k))$ 
		\Return $A_k$ \EndReturn
	 }\EndPart
	
	\Statex
	 \Part{Function: $\lit{isAbortable()}$ }{
		\If{$\exists X_j \in \Rset(T_k)$: $X_j\not\in \Wset(T_k)\wedge \Read(r_{j}) \neq 0$}
			\Return $\true$ \EndReturn
		\EndIf
		\If{$\exists X_j \in Rset(T_k)$:$[\textit{ov}_j,k_j]\neq \Read(v_j)$} 
			\Return $\true$ \EndReturn
		\EndIf
		\Return $\false$ \EndReturn
	}\EndPart
	\Statex
	\textbf{Code for fast-path transactions}
	\Part{$\textit{read}_k(X_j)$}\quad\Comment{fast-path}{
		\State $\textit{ov}_j := \Read(v_j)$ \Comment{uncached read} 
		
		\If{$r_{j}\neq 0$}  \Comment{Cached}		
			\Return $A_k$ \EndReturn
		\EndIf
		
		\Return $\textit{ov}_j$ \EndReturn
		
   	 }\EndPart
	\Statex
	\Part{$\textit{write}_k(X_j,v)$}{\quad\Comment{fast-path}
		\If{$r_{j}\neq 0$}  \Comment{Cached}		
			\Return $A_k$ \EndReturn
		\EndIf
		\State $\Write(v_j,\textit{nv}_j)$ \Comment{uncached write} 
		%\State $\ms{Increment}(c_j)$ \Comment{Uncached write}
		\Return $\ok$ \EndReturn
		
   	}\EndPart
	\Statex
	
	\Part{$\textit{tryC}_k$()}{\quad\Comment{fast-path}
		\State $\ms{commit-cache}_i$ 
  	 }\EndPart		
% 	
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm}

==> seq-hytm.tex <==
\begin{algorithm}[!h]
\caption{Opaque HyTM implementation with progressive slow-path and sequential fast-path TM-progress; code for $T_k$ by process $p_i$}
\label{alg:inswrite2}
\begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{
  	\footnotesize
	\Part{Shared objects}{
		\State $v_j \in \mathbb{D}$, for each t-object $X_j$ 
		\State ~~~~~allows reads, writes and cas
		%\State $L[i]$, a multi-trylock object for transaction $T_i$ 
		\State $r_{j} \in \mathbb{M}$, for each t-object $X_j$
		\State ~~~~~allows reads, writes and cas
		\State $\ms{fa}$, fetch-and-add object 
		%\State ~~~~~allows isEmpty, insert and remove
		%\State implemented from reads and writes
		%\State $L$, multi-trylock
	}\EndPart	
	
	\Statex	
	\textbf{Code for slow-path transactions}
	\Part{\TryC$_k$()}{\quad\Comment{slow-path}
		\If{$\Wset(T_k)= \emptyset$}
			\Return $C_k$  \EndReturn
		\EndIf
				
		\State locked := $\lit{acquire}(\Wset(T_k))$ 
		\If{$\neg$ locked} 
	 		\Return $A_k$ \EndReturn
	 	\EndIf
	 	\State $\ms{fa}.\lit{add}(1)$ 
		\If{$\lit{isAbortable}()$} 
			\State $\lit{release}( \ms{Lset}(T_k))$ 
			\Return $A_k$ \EndReturn
		\EndIf
		\ForAll{$X_j \in \Wset(T_k)$}
	 		 \If{ $v_j.\lit{cas}((ov_j, k_j),(\textit{nv}_j,k))$} 
			      \State $\ms{Oset}(T_k):=\ms{Oset}(T_k)\cup \{X_j\}$
			 \Else
			      \Return $\lit{undo}(\ms{Oset}(T_k))$ \EndReturn
			 \EndIf
			 
	 	\EndFor		
		\State $\lit{release}(\Wset(T_k))$ \label{line:rel2}
   		\Return $C_k$ \EndReturn
   	 }\EndPart		
	 
 	\newpage
 	
	 \Part{Function: $\lit{release}(Q)$}{
  		\ForAll{$X_j \in Q$}	
 			\State $r_j.\Write(0)$
		\EndFor
		\State $\ms{fa}.\lit{add}(-1)$ \label{line:dec}
		%\State $Rset_k:=Wset_k:=\emptyset$
		\Return \ok \EndReturn
	}\EndPart
	\Statex
	\Statex

	\textbf{Code for fast-path transactions}	
	
	\Part{$\textit{read}_k(X_j)$}{\quad\Comment{fast-path}
		\If{$Rset(T_k) = \emptyset$}
			\State $l \gets \Read(\ms{fa})$ \Comment{cached read} \label{line:fread}
		
			\If{$\ms{l}\neq 0$}
			    \Return $A_k$ \EndReturn
			\EndIf
		\EndIf
		\State $(\textit{ov}_j,k_j) := v_j.\Read()$ \Comment{cached read}
		
		\Return $\textit{ov}_j$ \EndReturn
		
   	 }\EndPart
	\Statex
	\Part{$\textit{write}_k(X_j,v)$}{\quad\Comment{fast-path}
		\State $v_j.\Write(\textit{nv}_j,k)$ \Comment{cached write} 
		\Return $\ok$ \EndReturn
		
   	}\EndPart
	\Statex
	
	%\Statex	
	\Part{$\textit{tryC}_k$()}{\quad\Comment{fast-path}
		%\Return $C_k$ \EndReturn
		\State $\ms{commit-cache}_i$ \Comment{returns $C_k$}
		
   		
   	 }\EndPart		
	
% 	
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm}


==> vlock-alg.tex <==
\begin{algorithm*}[ht]
\caption{Versioned lock}
\label{alg:vlock}
  \begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{\size
	
	\Part{Private field}{
		\State $r$, an integer initially $0$
	}\EndPart

	\Statex

	
% ------------- getVersion ---------------
	\Part{$\lit{getVersion}()$}{ \Comment {only return even value}
		\State {\bf return} $\ms{r}.\lit{read}()$ $\mathrel{\&}1111...1110$
	}\EndPart

	\Statex
	\Part{$\lit{isLocked}()$}{ \Comment {only return even value}
		\State {\bf return} $\ms{r}.\lit{read}()$ $\mathrel{\&}0000...0001$
	}\EndPart
	\Statex

% ------------- lockAtCurrentVersion ---------------
	\Part{Function: $\lit{setV}()$}{ \Comment{spin lock on the latest version}
		\State $\ms{success} \gets \lit{false}$
		
		\While{($\neg \ms{success}$)} \Comment {spin until we get the lock}
		\State $\ms{val} \gets$ $r.\Read()$ $\mathrel{\&}1111...1110$
		\State $\ms{success} \gets r$.CAS($val$, $val+1$)
		\EndWhile
	}\EndPart

% ------------- unlockAndIncrementVersion ---------------
	\Part{$\lit{unsetV}()$}{ \Comment{assuming already locked (odd value)}
		\State $\ms{val} \gets \ms{r}.\lit{read}()$
		\State $\ms{r}$.CAS($val$, $val+1$) 
	}\EndPart

	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}

